Vision-Language Models Do Not Understand Negation

Many practical vision-language applications require models that understand negation, e.g., when using natural language to retrieve images which contain certain objects but not others. Despite advancements in vision-language models (VLMs) through large-scale training, their ability to comprehend negation remains underexplored. This study addresses the question: how well do current VLMs understand negation? We introduce NegBench, a new benchmark designed to evaluate negation understanding across 18 task variations and $79$k examples spanning image, video, and medical datasets. The benchmark consists of two core tasks designed to evaluate negation understanding in diverse multimodal settings: Retrieval with Negation and Multiple Choice Questions with Negated Captions. Our evaluation reveals that modern VLMs struggle significantly with negation, often performing at chance level. To address these shortcomings, we explore a data-centric approach wherein we finetune CLIP models on large-scale synthetic datasets containing millions of negated captions. We show that this approach can result in a 10% increase in recall on negated queries and a 28% boost in accuracy on multiple-choice questions with negated captions.

==> sec/2_related_work_old.tex <==
\section{Related Work} 
\paragraph{Evaluating Negation Understanding.} 
Recent benchmarks show that language models (LMs) struggle with negation. \cite{garcia2023dataset} introduced a dataset for evaluating negation in LMs, finding that while LMs handle affirmative statements well, they generalize poorly to negation understanding. Extending this analysis to VLMs, we hypothesize that their negation understanding is likely worse due to fewer negation examples in their datasets, leading to weaker negation representations. As we show in \Cref{sec:mcq_why}, this lack of data leads to substantial affirmation bias, with models collapsing negated and affirmative captions into similar embeddings.

While CREPE \citep{ma2023crepe} is a vision-language model benchmark that includes a \textit{negation hard negatives (HN-NEG)} subset, its primary focus is on compositional understanding rather than negation specifically. 
% CREPE uses a templated approach, where negation is either applied to entire captions or specific objects. 
In contrast, our approach leverages an LLM to paraphrase negated captions into more natural-sounding sentences. As shown in \Cref{fig:mcq_breakdown}, this distinction is critical, as VLM behavior may change significantly when tested on natural paraphrases versus templated negations. We extend this analysis in \Cref{fig:caption_projection_pca}, where we show how CLIP-like models trained with different objectives develop distinct shortcut strategies. For example, some models generate nearly identical embeddings for captions with opposite meanings (e.g., ``there is a dog" vs. ``there is no dog"), effectively ignoring negation words like ``no" and ``without." In \Cref{sec:data_centric_solution}, we propose a synthetic data-centric fix that substantially reduces VLMs' reliance on these shortcuts, mitigating the affirmation bias and improving their understanding of negation.

\paragraph{Existing Methods for Multimodal Negation Understanding.}
CLIP \citep{radford2021learning} serves as a foundational vision-language model, known for its strong generalization abilities by aligning images and text through contrastive learning. NegCLIP \citep{yuksekgonul2023and} builds on CLIP by introducing composition-aware hard negative mining, which improves its ability to handle compositional tasks. However, our evaluations show that CLIP and NegCLIP struggle with negation, frequently collapsing affirmative and negated captions into similar embeddings. To address this issue, ConCLIP \citep{singh2024learn} modifies the CLIP loss and incorporates synthetically generated negated datasets. Despite its promise, we show in \Cref{fig:mcq_breakdown,fig:caption_projection_pca} that ConCLIP overfits to specific linguistic templates, limiting its performance on diverse and naturally phrased negations.

In the medical field, one can directly train a contrastive model on medical reports, which naturally contain negations \citep{tiu2022expert, boecking2022making, seibold2022breaking}. At inference time, these models use a simple presence (affirmative) prompt and absence (negative) prompt to detect the existence of a pathology. %While effective for improving multilabel classification (e.g., identifying pathologies), this approach does not directly test for negation understanding. 
This leverages negation as a feature in classification tasks, without evaluating whether the model comprehends the linguistic structure of negation itself. In contrast, our work focuses on assessing the impact of negation on VLM performance through the dedicated Retrieval-Neg and MCQ-Neg tasks. Our experiments reveal that even medical foundation models, which are trained on datasets that presumably include negations, exhibit a sharp decline in performance on the MCQ-Neg task.

\paragraph{Synthetic Data for Model Training.}
Recent works like StableRep \citep{tian2023stablerep}, SynCLR \citep{tian2024learning}, and SynthCLIP \citep{hammoud2024synthclip} show that models trained on synthetic data can achieve performance competitive with real data on standard vision tasks. However, they focus on general capabilities and do not address negation. Our work differs by using synthetic data to evaluate and fine-tune CLIP’s negation understanding, while maintaining general performance. Additionally, unlike prior methods that rely on explicit concept annotations, we leverage an LLM to extract concepts from captions, allowing us to generate datasets without manual labeling. 
